Convexified Open-Loop Stochastic Optimal Control for Linear Non-Gaussian Systems

We consider stochastic optimal control of linear dynamical systems with additive non-Gaussian disturbance. We propose a novel, sampling-free approach, based on Fourier transformations and convex optimization, to cast the stochastic optimal control problem as a difference-of-convex program. In contrast to existing moment based approaches, our approach invokes higher moments, resulting in less conservatism. We employ piecewise affine approximations and the well-known convex-concave procedure, to efficiently solve the resulting optimization problem via standard conic solvers. We demonstrate that the proposed approach is computationally faster than existing particle based and moment based approaches, without compromising probabilistic safety constraints.

==> arxiv v1/macrosv1.tex <==
% This file contains a collection of useful macros commonly used by the kinematics and robotics community. 

% Use the command "\input{macrosv1.tex}" to use them in a document. All the macros have been defined so that they can be called without using the math mode delimiter ($) and with xspace. 

%This is version - 1 of this document created on 5th March, 2015.
%-----------------------------------------------------------------------------------------------------
%-----------------------------------------------------------------------------------------------------

\usepackage{xspace}
\usepackage{amsmath,amssymb,amsfonts}

%-----------------------------------------------------------------------------------------------------

% Generic commands

%% Definition of mathmode bold symbols
\newcommand{\bs}[1]{\ensuremath{\boldsymbol{#1}}}
\newcommand{\mt}[1]{\ensuremath{{#1}}\xspace}

%-----------------------------------------------------------------------------------------------------

% Vector symbols: lower case English characters

\newcommand{\ba}{\ensuremath{\bs a}\xspace}
\newcommand{\bb}{\ensuremath{\bs b}\xspace}
\newcommand{\bc}{\ensuremath{\bs c}\xspace}
\newcommand{\bd}{\ensuremath{\bs d}\xspace}
\newcommand{\be}{\ensuremath{\bs e}\xspace}
\newcommand{\bsf}{\ensuremath{\bs f}\xspace}
\newcommand{\bg}{\ensuremath{\bs g}\xspace}
\newcommand{\bh}{\ensuremath{\bs h}\xspace}
\newcommand{\bi}{\ensuremath{\bs i}\xspace}
\newcommand{\bj}{\ensuremath{\bs j}\xspace}
\newcommand{\bk}{\ensuremath{\bs k}\xspace}
\newcommand{\bl}{\ensuremath{\bs l}\xspace}
\newcommand{\bm}{\ensuremath{\bs m}\xspace}
\newcommand{\bn}{\ensuremath{\bs n}\xspace}
\newcommand{\bo}{\ensuremath{\bs o}\xspace}
\newcommand{\bp}{\ensuremath{\bs p}\xspace}
\newcommand{\bq}{\ensuremath{\bs q}\xspace}
\newcommand{\br}{\ensuremath{\bs r}\xspace}
\newcommand{\bfs}{\ensuremath{\bs s}\xspace}
\newcommand{\bt}{\ensuremath{\bs t}\xspace}
\newcommand{\bu}{\ensuremath{\bs u}\xspace}
\newcommand{\bv}{\ensuremath{\bs v}\xspace}
\newcommand{\bw}{\ensuremath{\bs w}\xspace}
\newcommand{\bx}{\ensuremath{\bs x}\xspace}
\newcommand{\by}{\ensuremath{\bs y}\xspace}
\newcommand{\bz}{\ensuremath{\bs z}\xspace}

% Matrix symbols: upper case English characters

\newcommand{\bA}{\ensuremath{\bs A}\xspace}
\newcommand{\bB}{\ensuremath{\bs B}\xspace}
\newcommand{\bC}{\ensuremath{\bs C}\xspace}
\newcommand{\bD}{\ensuremath{\bs D}\xspace}
\newcommand{\bE}{\ensuremath{\bs E}\xspace}
\newcommand{\bF}{\ensuremath{\bs F}\xspace}
\newcommand{\bG}{\ensuremath{\bs G}\xspace}
\newcommand{\bH}{\ensuremath{\bs H}\xspace}
\newcommand{\bI}{\ensuremath{\bs I}\xspace}
\newcommand{\bJ}{\ensuremath{\bs J}\xspace}
\newcommand{\bK}{\ensuremath{\bs K}\xspace}
\newcommand{\bL}{\ensuremath{\bs L}\xspace}
\newcommand{\bM}{\ensuremath{\bs M}\xspace}
\newcommand{\bN}{\ensuremath{\bs N}\xspace}
\newcommand{\bO}{\ensuremath{\bs O}\xspace}
\newcommand{\bP}{\ensuremath{\bs P}\xspace}
\newcommand{\bQ}{\ensuremath{\bs Q}\xspace}
\newcommand{\bR}{\ensuremath{\bs R}\xspace}
\newcommand{\bS}{\ensuremath{\bs S}\xspace}
\newcommand{\bT}{\ensuremath{\bs T}\xspace}
\newcommand{\bU}{\ensuremath{\bs U}\xspace}
\newcommand{\bV}{\ensuremath{\bs V}\xspace}
\newcommand{\bW}{\ensuremath{\bs W}\xspace}
\newcommand{\bX}{\ensuremath{\bs X}\xspace}
\newcommand{\bY}{\ensuremath{\bs Y}\xspace}
\newcommand{\bZ}{\ensuremath{\bs Z}\xspace}

% Greek letters

%% Mathmode greek symbols, lower case
\newcommand{\alp}{\ensuremath{\alpha}\xspace}
\newcommand{\bet}{\ensuremath{\beta}\xspace}
\newcommand{\gm}{\ensuremath{\gamma}\xspace}
\newcommand{\del}{\ensuremath{\delta}\xspace}
\newcommand{\eps}{\ensuremath{\epsilon}\xspace}
\newcommand{\veps}{\ensuremath{\varepsilon}\xspace}
\newcommand{\zet}{\ensuremath{\zeta}\xspace}
\newcommand{\et}{\ensuremath{\eta}\xspace}
\newcommand{\tht}{\ensuremath{\theta}\xspace}
\newcommand{\vth}{\ensuremath{\vartheta}\xspace}
\newcommand{\iot}{\ensuremath{\iota}\xspace}
\newcommand{\kap}{\ensuremath{\kappa}\xspace}
\newcommand{\vkap}{\ensuremath{\varkappa}\xspace}
\newcommand{\lam}{\ensuremath{\lambda}\xspace}
\newcommand{\mmu}{\ensuremath{\mu}\xspace}
\newcommand{\mnu}{\ensuremath{\nu}\xspace}
\newcommand{\mxi}{\ensuremath{\xi}\xspace}
\newcommand{\omic}{\ensuremath{\omicron}\xspace}
\newcommand{\mpi}{\ensuremath{\pi}\xspace}
\newcommand{\vpi}{\ensuremath{\varpi}\xspace}
\newcommand{\mrho}{\ensuremath{\rho}\xspace}
\newcommand{\vrho}{\ensuremath{\varrho}\xspace}
\newcommand{\sig}{\ensuremath{\sigma}\xspace}
\newcommand{\vsig}{\ensuremath{\varsigma}\xspace}
\newcommand{\mtau}{\ensuremath{\tau}\xspace}
\newcommand{\ups}{\ensuremath{\upsilon}\xspace}
\newcommand{\ph}{\ensuremath{\phi}\xspace}
\newcommand{\vph}{\ensuremath{\varphi}\xspace}
\newcommand{\mchi}{\ensuremath{\chi}\xspace}
\newcommand{\mpsi}{\ensuremath{\psi}\xspace}
\newcommand{\om}{\ensuremath{\omega}\xspace}

%% Mathmode bold Greek symbols, lower case
\newcommand{\balp}{\ensuremath{\bs \alpha}\xspace}
\newcommand{\bbet}{\ensuremath{\bs \beta}\xspace}
\newcommand{\bgamma}{\ensuremath{\bs \gamma}\xspace}
\newcommand{\bdel}{\ensuremath{\bs \delta}\xspace}
\newcommand{\beps}{\ensuremath{\bs \epsilon}\xspace}
\newcommand{\bveps}{\ensuremath{\bs \varepsilon}\xspace}
\newcommand{\bzet}{\ensuremath{\bs \zeta}\xspace}
\newcommand{\bfeta}{\ensuremath{\bs \eta}\xspace}
\newcommand{\bth}{\ensuremath{\bs \theta}\xspace}
\newcommand{\bvth}{\ensuremath{\bs \vartheta}\xspace}
\newcommand{\biot}{\ensuremath{\bs \iota}\xspace}
\newcommand{\bkap}{\ensuremath{\bs \kappa}\xspace}
\newcommand{\bvkap}{\ensuremath{\bs \varkappa}\xspace}
\newcommand{\blam}{\ensuremath{\bs \lambda}\xspace}
\newcommand{\bmu}{\ensuremath{\bs \mu}\xspace}
\newcommand{\bnu}{\ensuremath{\bs \nu}\xspace}
\newcommand{\bxi}{\ensuremath{\bs \xi}\xspace}
\newcommand{\bomic}{\ensuremath{\bs \omicron}\xspace}
\newcommand{\bpi}{\ensuremath{\bs \pi}\xspace}
\newcommand{\bvpi}{\ensuremath{\bs \varpi}\xspace}
\newcommand{\brho}{\ensuremath{\bs \rho}\xspace}
\newcommand{\bvrho}{\ensuremath{\bs \varrho}\xspace}
\newcommand{\bsig}{\ensuremath{\bs \sigma}\xspace}
\newcommand{\bvsig}{\ensuremath{\bs \varsigma}\xspace}
\newcommand{\btau}{\ensuremath{\bs \tau}\xspace}
\newcommand{\bups}{\ensuremath{\bs \upsilon}\xspace}
\newcommand{\bphi}{\ensuremath{\bs \phi}\xspace}
\newcommand{\nvph}{\ensuremath{\bs \varphi}\xspace}
\newcommand{\bch}{\ensuremath{\bs \chi}\xspace}
\newcommand{\bpsi}{\ensuremath{\bs \psi}\xspace}
\newcommand{\bom}{\ensuremath{\bs \omega}\xspace}

%% Mathmode Greek symbols,upper case
\newcommand{\Gm}{\ensuremath{\Gamma}\xspace}
\newcommand{\Del}{\ensuremath{\Delta}\xspace}
\newcommand{\Th}{\ensuremath{\Theta}\xspace}
\newcommand{\Lam}{\ensuremath{\Lambda}\xspace}
\newcommand{\mXi}{\ensuremath{\Xi}\xspace}
\newcommand{\mPi}{\ensuremath{\Pi}\xspace}
\newcommand{\Sig}{\ensuremath{\Sigma}\xspace}
\newcommand{\Ups}{\ensuremath{\Upsilon}\xspace}
\newcommand{\Ph}{\ensuremath{\Phi}\xspace}
\newcommand{\Ps}{\ensuremath{\Psi}\xspace}
\newcommand{\Om}{\ensuremath{\Omega}\xspace}

%% Mathmode bold Greek symbols, upper case
\newcommand{\bGm}{\ensuremath{\bs \Gamma}\xspace}
\newcommand{\bDel}{\ensuremath{\bs \Delta}\xspace}
\newcommand{\bTh}{\ensuremath{\bs \Theta}\xspace}
\newcommand{\bLam}{\ensuremath{\bs \Lambda}\xspace}
\newcommand{\bXi}{\ensuremath{\bs \Xi}\xspace}
\newcommand{\bPi}{\ensuremath{\bs \Pi}\xspace}
\newcommand{\bSig}{\ensuremath{\bs \Sigma}\xspace}
\newcommand{\bUps}{\ensuremath{\bs \Upsilon}\xspace}
\newcommand{\bPhi}{\ensuremath{\bs \Phi}\xspace}
\newcommand{\bPsi}{\ensuremath{\bs \Psi}\xspace}
\newcommand{\bOm}{\ensuremath{\bs{\Omega}}\xspace}

% Vector/matrix "zero"
\newcommand{\bzero}{\ensuremath{\bs{0}}\xspace}

% Half
\newcommand{\half}{\ensuremath{\frac{1}{2}}\xspace}

%-----------------------------------------------------------------------------------------------------

%  Spaces symbols

\newcommand{\C}{\ensuremath{\mathbb{C}}\xspace}
\newcommand{\Cn}{\ensuremath{\mathbb{C}^n}\xspace}
\newcommand{\D}{\ensuremath{\mathbb{D}}\xspace}
\newcommand{\Dn}{\ensuremath{\mathbb{D}^n}\xspace}
\renewcommand{\Re}{\ensuremath{\mathbb{R}}\xspace} % latex2e
\newcommand{\Rn}{\ensuremath{\mathbb{R}^n}\xspace}
%\newcommand{\se}{\ensuremath{se(3)}\xspace}
%\newcommand{\ses}{\ensuremath{se^*(3)}\xspace}
%\newcommand{\SE}{\ensuremath{\mathbb{SE}(3)}\xspace}
%\newcommand{\so}{\ensuremath{so(3)}\xspace}
%\newcommand{\SO}{\ensuremath{\mathbb{SO}(3)}\xspace}


%% Notations for the configuration space
\newcommand{\conf}{\ensuremath{\mathcal{C}}\xspace}
\newcommand{\dimc}{\ensuremath{\textrm{dim(}\mathcal{C}}\textrm{)}\xspace}

%-----------------------------------------------------------------------------------------------------
% Jacobian matrices

%% Constraint Jacobian matrices
\newcommand{\jetaq}{\ensuremath{{\boldsymbol J}_{\bfeta\bq}}\xspace}
\newcommand{\jetath}{\ensuremath{{\bs J}_{\bfeta\bth}}\xspace}
\newcommand{\jetaphi}{\ensuremath{{\bs J}_{\bfeta\bphi}}\xspace}
\newcommand{\jetagamma}{\ensuremath{{\bs J}_{\bfeta\bgamma}}\xspace}
\newcommand{\jetapsi}{\ensuremath{{\bs J}_{\bfeta\bpsi}}\xspace}
\newcommand{\jphith}{\ensuremath{{\bs J}_{\bphi\bth}}\xspace}
\newcommand{\jpsith}{\ensuremath{{\bs J}_{\bpsi\bth}}\xspace}
\newcommand{\jgammath}{\ensuremath{{\bs J}_{\bgamma\bth}}\xspace}

\newcommand{\jqth}{\ensuremath{{\boldsymbol{J}}_{\bq\bth}}\xspace}
\newcommand{\jpq}{\ensuremath{{\boldsymbol{J}}_{\bp\bq}}\xspace}

\newcommand{\jpcth}{\ensuremath{\boldsymbol{J}_{\pc\bth}\xspace}}
\newcommand{\jpcphi}{\ensuremath{\boldsymbol{J}_{\pc\bphi}\xspace}}
\newcommand{\jpcq}{\ensuremath{\boldsymbol{J}_{\pc\bq}\xspace}}

\newcommand{\jfth}{\ensuremath{\boldsymbol{J}_{\bs{f}\bth}\xspace}}
\newcommand{\jfpsi}{\ensuremath{\boldsymbol{J}_{\bs{f}\bpsi}\xspace}}
\newcommand{\jfrts}{\ensuremath{\boldsymbol{J}_{\bs{f}\bs{r}_{ts}}\xspace}}
\newcommand{\jfpc}{\ensuremath{\boldsymbol{J}_{\bs{f}\bp_c}\xspace}}

\newcommand{\jpth}{\ensuremath{\boldsymbol{J}_{\boldsymbol{p\theta}}\xspace}}
\newcommand{\jpphi}{\ensuremath{\boldsymbol{J}_{\boldsymbol{p\phi}}\xspace}}

%% Angular velocity related
\newcommand{\jom}{\ensuremath{{\bs J}_{\bom}}\xspace}
\newcommand{\jomc}[1]{\ensuremath{{\boldsymbol J}_{\boldsymbol{\omega}_{c_#1}}}\xspace}
\newcommand{\jomth}{\ensuremath{{\bs J}_{\bom\bth}}\xspace}
\newcommand{\jomphi}{\ensuremath{{\bs J}_{\bom\bphi}}\xspace}
\newcommand{\jomeq}{\ensuremath{{\bs J}_{\bom}^{eq}}\xspace}
\newcommand{\jweq}{\ensuremath{{\bs J}_{\bs{w}}^{eq}}\xspace}

%% Linear velocity related
\newcommand{\jv}{\ensuremath{{\bs J}_{\bs v}}\xspace}
\newcommand{\jvp}{\ensuremath{{\bs J}_{{\bs v}{\bs p}}}\xspace}
\newcommand{\jvth}{\ensuremath{{\bs J}_{\bv\bth}}\xspace}
\newcommand{\jvphi}{\ensuremath{{\bs J}_{\bv\bphi}}\xspace}
\newcommand{\jveq}{\ensuremath{{\bs J}_{\bv}^{eq}}\xspace}
\newcommand{\jc}{\ensuremath{{\bs J}_{\bs c}}\xspace}
\newcommand{\jvpc}[1]{\ensuremath{\boldsymbol{J}_{{\boldsymbol{v}_{\boldsymbol{p}_{c_#1}}}}\xspace}}
\newcommand{\jcp}{\ensuremath{\bs{J}_{\bs{c}{\bp}}}\xspace}

%-----------------------------------------------------------------------------------------------------
% Kinematics

\newcommand{\rot}[2]{\ensuremath{{}^{#1}_{#2}{\boldsymbol{R}}}\xspace}%rotation matrix
\newcommand{\tran}[2]{\ensuremath{{}^{#1}_{#2}{\boldsymbol{T}}}\xspace}
\newcommand{\frm}[1]{\ensuremath{\{#1\}}\xspace} % frame number
\newcommand{\pc}{\ensuremath{\boldsymbol{p}_c}\xspace}
\newcommand{\pci}[1]{\ensuremath{\bs{p}_{\boldsymbol{c}_{i}}}\xspace}

%% Velocities
\newcommand{\vp}{\ensuremath{\bs{v}_{\boldsymbol{p}}}\xspace} % place with velocity commands
\newcommand{\vpc}[1]{\ensuremath{\bs{v}_{\boldsymbol{p}_{c_#1}}}\xspace}

%% Derivatives
\newcommand{\xd}{\ensuremath{\dot{x}}\xspace}
\newcommand{\xdd}{\ensuremath{\ddot{x}}\xspace}
\newcommand{\bqd}{\ensuremath{\dot{\boldsymbol{q}}}\xspace}
\newcommand{\bqdd}{\ensuremath{\ddot{\boldsymbol{q}}}\xspace}
\newcommand{\pcd}{\ensuremath{\dot{\boldsymbol{p}_c}}\xspace}

\newcommand{\bthd}{\ensuremath{\dot{\bs{\theta}}}\xspace}
\newcommand{\bthdd}{\ensuremath{\ddot{\bth}}\xspace}
\newcommand{\alphad}{\ensuremath{\dot \alpha}\xspace}
\newcommand{\psid}{\ensuremath{\dot{\psi}}\xspace}
\newcommand{\psidd}{\ensuremath{\ddot{\psi}}\xspace}
\newcommand{\phid}{\ensuremath{\dot{\phi}}\xspace}
\newcommand{\bPhid}{\ensuremath{\dot{\bs{\Phi}}}\xspace}
\newcommand{\bphid}{\ensuremath{\dot{\bs{\phi}}}\xspace}
\newcommand{\bpsid}{\ensuremath{\dot{\bs{\psi}}}\xspace}

%-----------------------------------------------------------------------------------------------------.
% Dynamics

\newcommand{\bMth}{\ensuremath{\bs{M_\theta}}\xspace}
\newcommand{\bCth}{\ensuremath{\bs{C_\theta}}\xspace}
\newcommand{\bGth}{\ensuremath{\bs{G_\theta}}\xspace}

\newcommand{\bin}{\ensuremath{\bs{I}_n}\xspace}
\newcommand{\Ith}{\ensuremath{I(\theta)}\xspace}

\newcommand{\bkp}{\ensuremath{\boldsymbol{K}_p}\xspace}
\newcommand{\bkv}{\ensuremath{\boldsymbol{K}_v}\xspace}

\newcommand{\bQnc}{\ensuremath{\boldsymbol{Q}^{nc}}\xspace}

%-----------------------------------------------------------------------------------------------------.
% Manipulators

\newcommand{\rrs}{\ensuremath{3}-\underline{R}RS\xspace}
\newcommand{\rps}{\ensuremath{3}-R\underline{P}S\xspace}
\newcommand{\upu}{\ensuremath{3}-U\underline{P}U\xspace}
%\newcommand{\map}{\mbox{MaPaMan}\xspace}
%\newcommand{\mapI}{\mbox{MaPaMan-I}\xspace}
%\newcommand{\mapII}{\mbox{MaPaMan-II}\xspace}
\newcommand{\rrr}{\ensuremath{3}-\underline{R}RR\xspace}
\newcommand{\rpr}{\ensuremath{3}-R\underline{P}R\xspace}

%-----------------------------------------------------------------------------------------------------

% Math Symbols

\renewcommand{\iff}{\ensuremath{\mathit{iff}}\xspace}
%\newtheorem{thm}{Theorem}[section]
%\newcommand{\implies}{\ensuremath{\Rightarrow \;}\xspace}
\def\QED{\ensuremath{\rule[0pt]{1.5ex}{1.5ex}}\xspace}
\def\proof{\noindent\hspace{2em}{\em Proof: }}
\def\endproof{\hspace*{\fill}~\QED\par\endtrivlist\unskip}
%\newcommand{\mathe}{\begin{verbatim}Mathematica\end{verbatim}\xspace}
%\newcommand{\define}{\ensuremath{\stackrel{\Delta}{=}}\xspace}
\newcommand{\elim}[1]{\ensuremath{\stackrel{\times #1}{\longrightarrow}}\xspace}

%% Operations
\newcommand{\adj}{\text{adj}}
\newcommand{\trace}{\text{tr}}

%%% Norm
\newcommand{\norm}[1]{\ensuremath{\| #1\|}\xspace}
\newcommand{\normd}[1]{\ensuremath{\| #1\|_d}\xspace}

%%% Partial derivative
\newcommand{\pd}[2]{\ensuremath{\frac{\partial #1}{\partial #2}}\xspace}
\newcommand{\dpd}[2]{\ensuremath{\dfrac{\partial #1}{\partial #2}}\xspace}

%%% Total derivative
\newcommand{\td}[2]{\ensuremath{\frac{d #1}{d #2}}\xspace}
\newcommand{\dtotder}[2]{\ensuremath{\dfrac{d #1}{d #2}}\xspace}

%%% Partial second derivative
\newcommand{\pdd}[2]{\ensuremath{\frac{\partial^2 #1}{\partial #2^2}}\xspace}

%%% Total second derivative
\newcommand{\tdd}[2]{\ensuremath{\frac{d^2 #1}{d #2^2}}\xspace}
\newcommand{\dsecder}[2]{\ensuremath{\dfrac{\partial^2 #1}{\partial #2^2}}\xspace}

%%% Scalar tripple product
\newcommand{\trip}[3]{\ensuremath{\left[#1, #2, #3\right]\xspace}}

%% Rank symbols
%\newcommand{\rank}[1]{\ensuremath{\mathrm{rank}\left(#1\right)}\xspace}

%-----------------------------------------------------------------------------------------------------

% Generic words

\newcommand{\dof}{degree-of-freedom\xspace}
\newcommand{\dofs}{degrees-of-freedom\xspace}
\newcommand{\rb}{rigid-body\xspace}
\newcommand{\rbm}{rigid-body motion\xspace}

%-----------------------------------------------------------------------------------------------------

